Multi-SIM support in 5G Evolution: Challenges and Opportunities

Devices with multiple Subscriber Identification Modules (SIM)s are expected to prevail over the conventional devices with only one SIM. Despite the growing demand for such devices, only proprietary solutions are available so far. To fill this gap, the Third Generation Partnership Project (3GPP) is aiming at the development of unified cross-platform solutions for multi-SIM device coordination. This paper extends the technical discussion and investigation of the 3GPP solutions for improving mobile Terminated (MT) service delivery to multi-SIM devices. Implementation trade-offs, impact on the Quality of Service(QoS), and possible future directions in 3GPP are outlined.

==> comparison.tex <==
\definecolor{green}{rgb}{0.62, 0.84, 0.43}%

\newcommand{\D}{5} % number of dimensions (config option)
\newcommand{\U}{6} % number of scale units (config option)
\newcommand\ColorBox[1]{\textcolor{#1}{\rule{2ex}{2ex}}}

\newdimen\R % maximal diagram radius (config option)
\R=3.5cm 
\newdimen\L % radius to put dimension labels (config option)
\L=4cm

\newcommand{\A}{360/\D} % calculated angle between dimension axes

\begin{tikzpicture}[scale=1]
  \path (0:0cm) coordinate (O); % define coordinate for origin

  % draw the spiderweb
  \foreach \X in {1,...,\D}{
    \draw (\X*\A:0) -- (\X*\A:\R);
  }

  \foreach \Y in {0,...,\U}{
    \foreach \X in {1,...,\D}{
      \path (\X*\A:\Y*\R/\U) coordinate (D\X-\Y);
      \fill (D\X-\Y) circle (1pt);
    }
    \draw [opacity=0.3] (0:\Y*\R/\U) \foreach \X in {1,...,\D}{
        -- (\X*\A:\Y*\R/\U)
    } -- cycle;
  }
%
  % define labels for each dimension axis (names config option)
  \path (1*\A:\L) node (L1) {Complexity};
  \path (2*\A:\L) node (L2) {Latency};
  \path (3*\A:\L) node (L3) {Scalability};
  \path (4*\A:\L) node (L4) {Energy efficiency};
  \path (5*\A:\L+6) node (L5) {Overhead};

  % for each sample case draw a path around the web along concrete values
  % for the individual dimensions. Each node along the path is labeled
  % with an identifier using the following scheme:
  %
  %   D<d>-<v>, dimension <d> a number between 1 and \D (#dimensions) and
  %             value <v> a number between 0 and \U (#scale units)
  %
  % The paths will be drawn half-opaque, so that overlapping parts will be
  % rendered in a composite color.

  % Example Case 1 (red)
  %
  % D1 (Security): 0/7; D2 (Content Quality): 5/7; D3 (Performance): 0/7;
  % D4 (Stability): 6/7; D5 (Usability): 0/7; D6 (Generality): 5/7;
  % D7 (Popularity): 0/7
  \draw [color=blue,line width=1.5pt,opacity=0.5,fill=blue]
    (D1-4) --
    (D2-4) --
    (D3-2) --
    (D4-3) -- 
    (D5-4) -- cycle;

  % Example Case 2 (green)
  %
  % D1 (Security): 2/7; D2 (Content Quality): 2/7; D3 (Performance): 5/7;
  % D4 (Stability): 1/7; D5 (Usability): 4/7; D6 (Generality): 1/7;
  % D7 (Popularity): 7/7
  \draw [color=red,line width=1.5pt,opacity=0.5,fill=red]
    (D1-2) --
    (D2-3) --
    (D3-4) --
    (D4-2) --
    (D5-2) -- cycle;
   
\node[anchor=south west,xshift=-70pt,yshift=20pt] at (current bounding box.south east) 
{
\begin{tabular}{@{}lp{3cm}@{}}
\ColorBox{blue!50} & RAN-based \\
\ColorBox{red!50} & CN-based \\
\end{tabular}
};
\end{tikzpicture}

